On Goodness of WiFi based Monitoring of Vital Signs in the Wild

WiFi channel state information (CSI) has emerged as a plausible modality for sensing different human vital signs, i.e. respiration and body motion, as a function of modulated wireless signals that travel between WiFi devices. Although a remarkable proposition, most of the existing research in this space struggles to withstand robust performance beyond experimental conditions. To this end, we take a careful look at the dynamics of WiFi signals under human respiration and body motions in the wild. We first characterize the WiFi signal components - multipath and signal subspace - that are modulated by human respiration and body motions. We extrapolate on a set of transformations, including first-order differentiation, max-min normalization and component projections, that faithfully explains and quantifies the dynamics of respiration and body motions on WiFi signals. Grounded in this characterization, we propose two methods: 1) a respiration tracking technique that models the peak dynamics observed in the time-varying signal subspaces and 2) a body-motion tracking technique built with a multi-dimensional clustering of evolving signal subspaces. Finally, we reflect on the manifestation of these techniques in a practical sleep monitoring application. Our systematic evaluation with over 550 hours of data from 5 users covering both line-of-sight (LOS) and non-line-of-sight (NLOS) settings shows that the proposed techniques can achieve comparable performance to purpose-built pulse-Doppler radar.

==> sections/breathingmotionandsleep.tex <==
\presec
\section{Relation of limb motion (activity) and breathing with sleep states}
\postsec

Motivate the intuition behind combining body movement + respiratory activity for multi-stage sleep monitoring.
%
[2014-Sleep-Wake Evaluation from Whole-Night Non-Contact Audio Recordings of Breathing Sounds] \cite{dafna2015sleep}
%
[2015 On the analysis and classification of sleep stages from cardiorespiratory activity \cite{long2015analysis}]
%
[2015 Sleep stage classification with ECG and respiratory effort] \cite{fonseca2015sleep}
%
[2012] Sleep-stage decision algorithm by using heartbeat and body-movement signals \cite{kurihara2012sleep}. 78\% average accuracy.
%
Breathing rate and consistency: breathing features capture and quantify variations in breathing periodicity as they contribute to distinguishing between sleep and wake epochs.
%

It was well established that changes in vigilance states strongly affect breathing rate and regularity in humans and animals.
%
Relation of body and limb motion with sleep quality and stages, sleep actigraphy \cite{sadeh1995role,sadeh2002role, ancoli2003role}.
%
Relation of respiration/breathing with sleep quality and stages \cite{douglas1982respiration, krieger1990breathing, long2014analyzing, long2014sleep}.
%
``In addition, respiratory dynamics,
such as respiratory frequency (breathing rate, BR) [C], respiratory variability [C], and respiratory
regularity [C], have also been proven to vary over sleep stages. This means that respiratory activity can be in turn used to separate sleep stages. Combining body movements
with cardiorespiratory activity can result in a superior sleep/wake performance [C\cite{long2015analysis}]. By
means of cardiac and/or respiratory signals, numerous papers were published aiming at different
classification tasks, such as the classification between sleep and wake [C\cite{long2015analysis}], between wake, REM sleep, and NREM sleep [C\cite{long2015analysis}], between wake, REM sleep, light
sleep, and SWS [C\cite{long2015analysis}], between REMsleep and NREMsleep [C\cite{long2015analysis}], between light sleep
and SWS [C\cite{long2015analysis}], between SWS and all the other sleep stages [C\cite{long2015analysis}], and even between full
sleep stages (wake, REM sleep, S1 sleep, S2 sleep, and SWS) [C\cite{long2015analysis}]. Note that some
of those studies executed several different sleep stage classification tasks and some made also
use of information about body movements." [C\cite{long2015analysis}]
%
Temporal patterns associated with sleep stages, govern the progression of light and deep sleep. Probability of deep sleep decreases as sleep progresses \cite{carskadon2005normal}.
